Autoregressive Perturbations for Data Poisoning

The prevalence of data scraping from social media as a means to obtain datasets has led to growing concerns regarding unauthorized use of data. Data poisoning attacks have been proposed as a bulwark against scraping, as they make data "unlearnable" by adding small, imperceptible perturbations. Unfortunately, existing methods require knowledge of both the target architecture and the complete dataset so that a surrogate network can be trained, the parameters of which are used to generate the attack. In this work, we introduce autoregressive (AR) poisoning, a method that can generate poisoned data without access to the broader dataset. The proposed AR perturbations are generic, can be applied across different datasets, and can poison different architectures. Compared to existing unlearnable methods, our AR poisons are more resistant against common defenses such as adversarial training and strong data augmentations. Our analysis further provides insight into what makes an effective data poison.

==> figures/plot-adversarial-training-defense.tex <==
\pgfplotsset{
    legend cell align=left,
}

\begin{figure}[t]
    \centering
    

\resizebox{0.5\linewidth}{0.4\linewidth}{%
\begin{tikzpicture}
\begin{axis}[
    xlabel={$\rho_a$},
    ylabel={CIFAR-10 Test Accuracy},
    xmin=0.125, xmax=0.75,
    ymin=20, ymax=100,
    xtick={0.125,0.25,0.5,0.75},
    ytick={40,60,80,100},
    legend pos=south east,
    legend style={nodes={scale=0.8, transform shape}, xshift=-8, yshift=8},
    ymajorgrids=true,
    grid style=dashed,
]
% Clean
\addplot[
    color=black,
    dashed,
    mark=o,
    mark size=2.5pt
    ]
    coordinates {
    (0.125, 87.07)
    (0.25, 84.75)
    (0.5, 81.19)
    (0.75, 77)
    };

% Error-Max
\addplot[
    color=green,
    mark=*, 
    mark size=2.5pt
    ]
    coordinates {
    (0.125, 33.33)
    (0.25, 71.69) 
    (0.5, 79.16)
    (0.75, 74.94)
    % (1, 79.67)
    };

% Error-Min
\addplot[
    color=blue,
    mark=+,
    mark size=2.5pt
    ]
    coordinates {
    (0.125, 71.05)
    (0.25, 83.18)
    (0.5, 81.18)
    (0.75, 77.21)
    };

% R4 
\addplot[
    color=orange,
    mark=asterisk,
    mark size=2.5pt
    ]
    coordinates {
    (0.125, 74.55)
    (0.25, 81.27)
    (0.5, 79.73)
    (0.75, 76.88)
    };    

% R16
\addplot[
    color=cyan,
    mark=oplus,
    mark size=2.5pt
    ]
    coordinates {
    (0.125, 48.12)
    (0.25, 71.24)
    (0.5, 80.37)
    (0.75, 76.59)
    };
    
% Random
\addplot[
    color=brown,
    mark=x,
    mark size=2.5pt
    ]
    coordinates {
    (0.125, 86.45)
    (0.25, 84.42)
    (0.5, 80.02)
    (0.75, 76.16)    
    };
    
% Autoregressive
\addplot[
    color=red,
    mark=triangle*,
    mark size=2.5pt
    ]
    coordinates {
    (0.125, 33.65)
    (0.25, 56.22) 
    (0.5, 80.15)
    (0.75, 76.72)
    % (1, 81.34)
    };
    

    \legend{Clean, Error-Max, Error-Min, Regions-4, Regions-16, Random, AR}
\end{axis}
\end{tikzpicture}
}
\caption{\textbf{Adversarial training.} CIFAR-10 test accuracy after adversarially training a RN-18 with different radii $\rho_a$, using a 7-step $\ell_2$ PGD attack. AR poisons remain effective at relatively larger radius.}
\label{fig:plot-adversarial-training-defense}
\end{figure}

==> tables/clean_mix_adv_train.tex <==
\begin{table}[t]
%   \caption{\textbf{Dataset independence.} AR noises are effective across a variety of datasets. We display clean test accuracy of RN-18 when training using standard augmentations on different dataset poisons, where clean images are perturbed within an $\ell_2$ ball of size $\epsilon = 1$.}
  \begin{minipage}[t]{.53\textwidth}%
  \caption{\textbf{Mixing Poisons with Clean Data.} CIFAR-10 test accuracy when a proportion of clean data is used in addition to a poison. Top row shows test accuracy when training on only the clean proportion of the data; \ie no poisoned data is used.}
  \vspace{2mm}
  \label{table-clean-mix}
  \centering
  \resizebox{\textwidth}{!}{
  \begin{tabular}[t]{lccccc}
    \toprule
    & \multicolumn{5}{c}{Clean Proportion} \\
    % \textbf{Noise | Clean Proportion}
    & 40\% & 30\%  & 20\%  &  10\% & 5\%   \\
    \midrule \midrule
    Clean Only          & 90.84 & 89.92 & 87.90 & 81.01 & 74.97  \\
    \midrule
    $\bullet$ Error-Max \cite{fowl2021adversarialpoison} & 88.51 & 87.09 & 83.68 & 81.72 & 75.66  \\
    $\bullet$ Error-Min \cite{huang2021unlearnable}      & 88.76 & 86.96 & 83.78 & 79.1 & 68.35  \\
    $\circ$ Regions-4 & 87.66 & 87.86 & 83.60 & 77.18 & 70.85  \\
    $\circ$ Regions-16 & 87.52 & 87.16 & \textbf{82.94} & 77.38 & \textbf{65.73}   \\
    $\circ$ Random Noise & 88.72 & 87.28 & 83.24 & 79.06 & 69.83  \\
    $\bullet$ AR (Ours) & \textbf{87.52} & \textbf{84.97} & 84.14 & \textbf{75.07} & 66.15 \\ 
    \bottomrule
  \end{tabular}
  }
  \end{minipage}%
  \hfill
  \begin{minipage}[t]{.45\textwidth}
  \caption{\textbf{Adversarial Training.} CIFAR-10 test accuracy after adversarially training with different radii $\rho_a$. Top row shows performance of adversarial training on clean data. AR poisons remain effective for small $\rho_a$.}
  \vspace{2mm}
  \label{table-adv-train}
  \centering
  \resizebox{\textwidth}{!}{
  \begin{tabular}[t]{lcccc}
    \toprule
    & \multicolumn{4}{c}{$\rho_{a}$} \\
    % \textbf{Noise | Clean Proportion}
    & 0.125 & 0.25  & 0.50  &  0.75 \\%\% & 5\% & 0\% \\
    \midrule \midrule
    Clean Data  & 87.07 & 84.75 & 81.19 & 77.01 \\ \midrule
    % $\bullet$ Error-Max \cite{fowl2021adversarialpoison} & $33.30_{\pm0.14}$ & $72.27_{\pm2.18}$ & $81.15_{\pm3.58}$ & $78.73_{\pm4.20}$ \\
    $\bullet$ Error-Max \cite{fowl2021adversarialpoison} & \textbf{33.33} & 71.69 & \textbf{79.16} & \textbf{74.94} \\
    $\bullet$ Error-Min \cite{huang2021unlearnable} & 71.05 & 83.18 & 81.18 & 77.21\\
    $\circ$ Regions-4 & 74.55 & 81.27 & 79.73 & 76.88\\
    $\circ$ Regions-16 & 48.12 & 71.24 & 80.37 & 76.59\\
    $\circ$ Random Noise & 86.45 & 84.42 & 80.02 & 76.16 \\
    $\bullet$ AR (Ours) & 33.65 & \textbf{56.22} & 80.15 & 76.72 \\
    \bottomrule
  \end{tabular}
  }
  \end{minipage}%
\end{table}




==> tables/defense-evaluations-simclr.tex <==
\begin{table}[h]
  \caption{\textbf{Self-supervised learning.} Clean CIFAR-10 test accuracy of SimCLR RN-50 using linear evaluation. For error-maximizing, error-minimizing, and AR poisons, images are images are perturbed within an $\ell_2$ ball of size $\epsilon=1$.}
  \label{table-defense-evaluations-simclr}
  \centering
  \begin{tabular}{lcc}
    \toprule
                           &  Acc ($\downarrow$)  \\
    \midrule
    Clean Train            & 93.30 \\        
    Error-Max \cite{fowl2021adversarialpoison}      & 68.30 \\
    Error-Min \cite{huang2021unlearnable}      & - \\
    Autoregressive (Ours)  & 81.60 \\
    \bottomrule
  \end{tabular}
\end{table}

% TODO: Big caveat on Error-Max eps=1.0 is that the eps is really around 1.2, due to crafting this noise in normalized image space

